Long Polynomial Modular Multiplication using Low-Complexity Number Theoretic Transform

This tutorial aims to establish connections between polynomial modular multiplication over a ring to circular convolution and discrete Fourier transform (DFT). The main goal is to extend the well-known theory of DFT in signal processing (SP) to other applications involving polynomials in a ring such as homomorphic encryption (HE). HE allows any third party to operate on the encrypted data without decrypting it in advance. Since most HE schemes are constructed from the ring-learning with errors (R-LWE) problem, efficient polynomial modular multiplication implementation becomes critical. Any improvement in the execution of these building blocks would have significant consequences for the global performance of HE. This lecture note describes three approaches to implementing long polynomial modular multiplication using the number theoretic transform (NTT): zero-padded convolution, without zero-padding, also referred to as negative wrapped convolution (NWC), and low-complexity NWC (LC-NWC).

==> 99_bio.tex <==


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.33in,clip]{Chiu.jpg}}]{Sin-Wei Chiu} (Graduate Student Member, IEEE) 
received his bachelor’s degree in electrical engineering from National Central University, Taiwan, in 2020. He is currently pursuing a Ph.D. degree in electrical engineering at the University of Minnesota, Twin Cities. His current research interests include VLSI architecture design, digital signal processing systems, post-quantum cryptography, and homomorphic encryption. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.26in,clip]{parhi.jpg}}]{Keshab K. Parhi} (Fellow, IEEE) is the Erwin A. Kelen Chair in Electrical Engineering and a Distinguished McKnight University Professor in the Department of Electrical and Computer Engineering. He completed his Ph.D. in EECS at the University of California, Berkeley in 1988. He has published over 700 papers, is the inventor of 34 patents, and has authored the textbook VLSI Digital Signal Processing Systems (Wiley, 1999). His current research addresses VLSI architectures for machine learning, hardware security, data-driven neuroscience and DNA computing. Dr. Parhi is the recipient of numerous awards including the 2003 IEEE Kiyo Tomiyasu Technical Field Award, and the 2017 Mac Van Valkenburg award and the 2012 Charles A. Desoer Technical Achievement award from the IEEE Circuits and Systems Society. He served as the Editor-in-Chief of the {\em IEEE Trans. Circuits and Systems, Part-I: Regular Papers} during 2004 and 2005. He is a Fellow of the ACM, AIMBE, AAAS, and NAI.
\end{IEEEbiography}

==> Response.tex <==
\onecolumn
\pagenumbering{arabic} 



% % This refines the format of how the reviewer/point reference will appear.
% \renewcommand{\thepoint}{P\,\thereviewer.\arabic{point}} 

% % command declarations for reviewer points and our responses
% \newcommand{\reviewersection}{\stepcounter{reviewer} \bigskip \hrule
%                   \section*{Reviewer \thereviewer}}

% \newenvironment{point}
%    {\refstepcounter{point} \bigskip \noindent {\textbf{Reviewer~Point~\thepoint} } ---\ }
%    {\par }

% \newcommand{\shortpoint}[1]{\refstepcounter{point}  \bigskip \noindent 
% 	{\textbf{Reviewer~Point~\thepoint} } ---~#1\par }

% \newenvironment{reply}
%    {\medskip \noindent \begin{sf}\textbf{Reply}:\  }
%    {\medskip \end{sf}}

% \newcommand{\shortreply}[2][]{\medskip \noindent \begin{sf}\textbf{Reply}:\  #2
% 	\ifthenelse{\equal{#1}{}}{}{ \hfill \footnotesize (#1)}%
% 	\medskip \end{sf}}



\section*{Response to the reviewers}

The authors appreciate the numerous constructive comments from the two reviewers. All comments have been incorporated in the revised version. A list of changes is summarized below.

% \textcolor{red}{Summarize}

\begin{enumerate}
    \item Modification in Section \ref{secsco} and \ref{secrel} to increase readability.
    \item A new optimized version of the LC-INTT is added the the manuscript (denoted as Alt-LC-INTT) and comparisons with the standard LC-INTT are presented in Section \ref{secwhat}.
    \item Several updates on the figures in the manuscript.
\end{enumerate}

\reviewersection

\textbf{Summary}


The authors have successfully applied most of my recommendations. On
the one hand, in my opinion the manuscript has improved a lot
regarding how the topic is introduced to the SPM audience. On the
other hand, I also think there is still room for improvement in its
readability, and I recommend the authors to do a careful pass through
the document to make the text smoother and clearer, mainly in the
first pages.


\textbf{Areas for improvement}

After checking this new version, I also have some additional comments.
First, I include some parts where I think the explanations can be made
more accurate:

\begin{point}
    To be more precise in the number of multiplications required to homomorphically compute a function, I think it is useful to use "the multiplicative depth and width" defined here https://eprint.iacr.org/2020/1483 (in page 26). I say this because, while it is true that, in general, higher multiplicative depth implies a bigger number of multiplications, in some specific cases you could have more multiplications in circuits with smaller depth but much larger width. For example, consider $f(input) = input^8$, and $f(input) = input^6 + input^5 + input^4 + input^3 + input^2$. The first can be computed with only 3 multiplications, while the second one requires more multiplications).
\end{point}

\begin{reply}
    We agree with the reviewer's comment. It is more accurate to use ``the multiplicative depth and width". We have added the citation of the reference mentioned by the reviewer in Section \ref{secrel} when the multiplicative depth and width are mentioned.
\end{reply}


\begin{point}
     In the sentences "The ciphertexts of those schemes are in the form of polynomials. Therefore, the most time- and memory-Modular consuming part of an R-LWE-based scheme is the long polynomial modular multiplication." $=>$ it seems like there's a jump in the argument. You should also explain that homomorphic additions and multiplications require as building blocks the computation of additions and multiplications between the polynomials that form the ciphertexts.
\end{point}

\begin{reply}
    We agree that this paragraph needs more explanation. We have added a few more sentences to explain why the polynomial modular multiplication is the most time- and memory-consuming part of the R-LWE-based HE scheme in Section \ref{secrel}.  Thank you for your valuable comment.
\end{reply}

\textbf{Specific comments and corrections}

I include some general typos and mistakes I have detected in the examples through the document. Again, it is possible I have missed some of them, so I recommend the authors to do a careful pass.

\begin{point}
    \begin{enumerate}
        \item toward efficient NTT-base polynomial $=>$ "NTT-based"
        \item "Remember that DFT implements the circular convolution and to implement standard convolution, one needs to zero-pad two sequences for matching computation." $=>$ “Remember that with the DFT we can implement both circular and standard convolutions. For standard convolutions, it is necessary to zero-pad the two input sequences to ensure proper computation.”
        \item  "In these notes, we intend to extend the connection" $=>$ In these notes, we intend to provide a comprehensive explanation of the connection between ... with polynomial multiplication in …
        \item "is carried out in a ring [6], i.e., ..." $=>$ is carried out in a finite ring [6] working with an integer root of unity, i.e., …
        \item the Nth root of unity $=>$ the complex N-th root of unity.
        \item change the size of the matrices and vectors from "n by 1" and "n by n" to "n-by-1" and "n-by-n".
        \item The matrix W in page 2 $=>$ The element in position (4,4) is not 13, it should be 4. The rest of the values seem to be OK.
        \item The matrix $W^-1$ in page 2 $=>$ The element in position (4,4) is not 4, it should be 13.
        \item Page 2, column 2: "before modular reduction will be [494 308 377 293]. $=>$ It should be [494 4745 3029 4628].
        \item Page 3, column 1: Change "can't" by "cannot".
        \item Figure 1.(a). Shouldn't this figure include the zero-padding? 
        \item  Page 4, column 2: "For k = 0, 1, ..., n/2 - 1:" That expression seems to work also for k = 0, 1, ..., n - 1, and it must be particularized to two halves afterwards at the end of the page.
        \item Page 5, column 2: "For k = 0, 1, ..., n/2 - 1:" $=>$ it should be "k = 0, 1, ..., n - 1:" referring to $p_k$. The division in two parts is applied afterwards with the "2*k" and "2*k + 1" substitution over $p_{2k}$ and $p_{2k + 1}$.
        \item Page 6, column 2: "floor(x/2) in can be implemented" $->$ remove "in".
    \end{enumerate}
\end{point}

\begin{reply}
    Thank you for your comments and corrections. All mistakes have been corrected. In point number 9, the reviewer's comment and the original manuscript are both correct. [494 308 377 293] is the result of the multiplication of $\mathbf{W}^{-1} \mod{q}$ and $\mathbf{A}$. [494 4745 3029 4628] is the result of the multiplication of $\mathbf{W}^{-1}$ and $\mathbf{A}$. We have included the result of $\mathbf{W}^{-1} \mod{q}$ to clarify this issue.
\end{reply}

\textbf{Typos in the numerical example section:}

\begin{point}
    \begin{enumerate}
        \item Figure 3 INTT block: In the first line of the butterfly for $\tilde{P}_0$, you have: 15 15 10 15 16 16 15 15 4 $->$ the 10 should be "15".
        \item Page 7, column 1: "Let's consider the same example that both a(x) and b(x) are $4x^3 + 3x^2 + 2x + 1$." $=>$ the polynomial should be $"x^3 + 3x^2 + 4x + 2"$.
        \item Page 7, column 1: "We can verify this result by computing $(x^3 + 3x^2 + 4x + 2)^2$ mod $(x^4 + 1, 17) = x^6 + 6x^5 + 11x^3 + 11x^2 + 16x + 4$"$=->$ You are applying the mod 17 beforehand, maybe it is better to include it before reducing mod 17, which I think would be "$x^6 + 6x^5 + 17x^4 + 28x^3 + 28x^2 + 16x + 4$".
        \item Page 7, column 2: "The above comparison has taken multipliers that multiply..." $=>$ you do not explicitly cite Table II in the document.
        \item Page 8: Tables III and IV say the same method "convolution method" $=>$ Shouldn't it be zero-padding with NTT?
    \end{enumerate}
\end{point}

\begin{reply}
    Thank you for your feedback. All typos pointed out by the reviewer have been examined and addressed.
\end{reply}


\textbf{Possible novel improvements? A faster approach than LC-NTT/INTT by means of ``optimized1 and optimized2 NWC".}

\begin{point}
    I was suspecting this when suggesting to study how many multipliers were equal to "1", but I think that with a careful design, a new algorithm can be presented which is faster in terms of "operations" than the LC-NTT/INTT described in the manuscript. I detail the required modifications below:

    If we exclude multiplications with 1, the NWC has for the NWC-NTT $\frac{n}{2}log(n)$ multipliers, and for the NWC-INTT $\frac{n}{2}log(n) + n$ multipliers. However, in the NWC-INTT there are ``$n - 1$" multiplications with "$n^{-1}$" which can be directly combined with the postprocessing, so finally having multipliers with post processing "post $= n^{-1}\psi \mod q$".
    
    By doing this we can remove ``$n - 1$" multipliers, then having a total of only ``$\frac{n}{2}log(n) + 1$ multipliers" for the NWC-INTT. This trick cannot be applied in the first "line" of the butterfly because the post-processing is "1" there.

    Comparing now this with the LC-NWC:
    \begin{enumerate}
        \item optimized1 NWC-INTT has $\frac{n}{2}log(n) + 1$ multipliers
        \item LC-NWC INTT has $\frac{n}{2}log(n)$ multipliers $+ nlog(n)$ shift operations.
    \end{enumerate}

    While it is true that "optimized1" NWC-INTT has 1 multiplier more, the number of shift operations IN LC-NWC-INTT grows with "n", so asymptotically, optimized1 NWC-INTT should be more efficient.

    Alternatively, and similarly to what is done in LC-NWC, we could decompose the multiplier of the "first line" into $log(n)$ shifts. This means that we would have:

    \begin{enumerate}
        \item optimized2 NWC-INTT $=> \frac{n}{2}log(n)$ multipliers $+ log(n)$ shifts.
    \end{enumerate}

    This last option has the same number of multipliers as LC-NWC-INTT, and requires n times less shifts than LC-NWC-INTT.
    
    Another aspect worth mentioning is that the post-processing and pre-processing of the NWC-NTT/INTT can be easily parallelized as they correspond to "$n - 1$" independent multiplications. However, the multipliers in the LC-NWC-INTT/NTT are divided in consecutive layers which depend on the results of previous layers, not being as easy to parallelize.
\end{point}

\begin{reply}
    Thank you for this insightful feedback. We agree that there are advantages to the optimized-1 method suggested above. We have included an additional subsection in Section \ref{secso} to discuss the optimized-1 method (we addressed it as the alternative LC-INTT). Also in Section \ref{secwhat}, we have included a new table to give a complete comparison between the standard LC-INTT and the alternative LC-INTT methods.
    For the optimized-2 method suggested by the reviewer, there would be some issues when only decomposing the multiplier of the "first line" into $log(n)$ shifts. Since the computations of the later stage in the INTT are fully dependent on the prior stages, applying $2^{-1}$ to one of the signals in the early stages will not only change the output of $p_0$ but also the other outputs. 
    
\end{reply}
